Rebalancing Social Feed to Minimize Polarization and Disagreement

Social media have great potential for enabling public discourse on important societal issues. However, adverse effects, such as polarization and echo chambers, greatly impact the benefits of social media and call for algorithms that mitigate these effects. In this paper, we propose a novel problem formulation aimed at slightly nudging users' social feeds in order to strike a balance between relevance and diversity, thus mitigating the emergence of polarization, without lowering the quality of the feed. Our approach is based on re-weighting the relative importance of the accounts that a user follows, so as to calibrate the frequency with which the content produced by various accounts is shown to the user. We analyze the convexity properties of the problem, demonstrating the non-matrix convexity of the objective function and the convexity of the feasible set. To efficiently address the problem, we develop a scalable algorithm based on projected gradient descent. We also prove that our problem statement is a proper generalization of the undirected-case problem so that our method can also be adopted for undirected social networks. As a baseline for comparison in the undirected case, we develop a semidefinite programming approach, which provides the optimal solution. Through extensive experiments on synthetic and real-world datasets, we validate the effectiveness of our approach, which outperforms non-trivial baselines, underscoring its ability to foster healthier and more cohesive online communities.

==> notes.tex <==
\spara{GD-based method}
Gradient-based approaches are first-order methods that rely on computing the gradient of the objective function and updating the solution with a small increment in the opposite direction of the gradient. When the variable is a vector and the gradient is Lipschitz, the optimal learning rate is proportional to its inverse.


Here we follow the standard approach for vector-variables, and derive analytically the gradient  w.r.t the matrix $L$, furthermore we compute an upper bound of the Lipschitz constant.

\spara{Gradient.}
The gradient of the objective function in Eq. \ref{eq:problem}  w.r.t the graph structures is described by the following lemma.
 \begin{lemma}
 The gradient of $f(L):=s^T(I+L)^{-1}s$ w.r.t $L$ is
 \begin{equation}
     \partial_L f(L) := \partial_L  \mathcal{L}(L; Y)=-(I+L)^{-1}ss^T (I+L)^{-1}
     \label{eq:gradient}
 \end{equation}
 \end{lemma}
 \spara{Proof:}
  given $\partial_L (s^T (I + L)^{-1}s)$, \\
     we write its differential
         \begin{align*}
             d f(L)= d(s^T (I+L)^{-1} s) \\
             = d(Tr(s^T (I+L)^{-1} s)) \\
             = Tr(ss^T d(I+L)^{-1}))\\
             = Tr(-ss^T (I+L)^{-1}dL(I+L)^{-1}))\\
             = Tr(-(I+L)^{-1}ss^T (I+L)^{-1}dL)\\
         \end{align*}
          where we used: i. the trace of a scalar is a scalar, ii. trace cyclic property, and iii. $d (I+L)^{-1}=-(I+L)^{-1} dL (I+L)^{-1}$ \cite{petersen2008matrix}. Finally, using the derivative of a trace ($\partial_X Tr(AX)=A$),
         \[
         \partial_L f(L)=\partial_L (s^T (I + L)^{-1}s)= -(I+L)^{-1} ss^T (I+L)^{-1}
         \]\qedsymbol{}
\\
 \textit{Remark 1}: Due to the sum of the identity matrix $I$, the gradient and the objective are continuous in $L$.
 \\
 \textit{Remark 2}: Some entries of $L$ are constant and equal to zero due to the constraint of the feasible set in Eq. \ref{eq:feasible-set}, therefore their differential $dL_{ij}=0 \; \forall i,j \: s.t. \: A_{ij}=0$.
 \\
 \textit{Remark 3}: Letting $z=(I+L)^{-1}s$, the gradient is a rank-one matrix given by the external product $\partial_L f(L)=z z^T$. This implies that we can avoid the matrix inversion and solve directly the linear system $(I+L)z=s$ using a linear solver. As in \cite{marumo2021projected}, we prefered the Biconjugate Gradient (BiCG) solver \cite{fletcher1976numerical} to other solvers (LAPACK POSV routine\footnote{https://netlib.org/lapack/}, and Laplacian solver\footnote{https://github.com/danspielman/Laplacians.jl}) to exploit the sparsity of the matrix and to instantiate the solver at each iteration.



 \spara{Learning rate.}
There are various methods available to set the learning rate in gradient descent. In the unconstrained setting with a vector variable, when dealing with a convex function that has a $C$-Lipschitz-continuous gradient, convergence is achievable with a step size smaller than $1/C$, and the convergence rate is $\mathcal{O}(1/k)$ for $k$ iterates. Adaptive learning schemes such as ADAM and NAG are commonly used to attain superlinear convergence rates. To take into account the size of the constraint, recent approaches involve rescaling the learning rate using the diameter of the feasible set of solutions \cite{ene2021adaptive}.

In this problem, we are facing a constrained matrix-valued objective function, and we empirically compare two approaches: a fixed learning rate schedule based on the derived upper bound of the Lipschitz constant of the gradient and an adaptive learning rate.

The Lipschitz constant of our objective is described by the following lemma:

 \begin{lemma}
 The gradient of the matrix-valued objective function has a Lipschitz constant $C$ equal to $||s||^2$ w.r.t the spectral norm.
 \end{lemma}
 \spara{Proof:} We want to find the smallest $C$ such that
 \[
 ||\partial f(L + H) - \partial f(L)|| \leq C ||H||
 \]
 where $H=L_1-L_2$. We start from the left side,
 \begin{align*}
     ||\partial f(L+H) - \partial f(L)|| = ||  -(I+L+H)^{-1} s s^T(I+L+H)^{-1} + \\ + (I+L)^{-1}ss^T(I+L)^{-1}||
 \end{align*}
 using $(X+H)^{-1}=X^{-1}-X^{-1}HX^{-1}+ O(||H||^2)$, with $X=I+L$ and denoting $\Omega=(I+L)^{-1}$,
 \[
 \cong ||-(\Omega - \Omega H \Omega)ss^T(\Omega - \Omega H \Omega) + \Omega ss^T\Omega||
 \]
 \begin{equation}
 \cong ||-\Omega ss^T\Omega + \Omega ss^T \Omega H \Omega+ \Omega H \Omega ss^T\Omega+ \Omega ss^T\Omega||
 \label{eq:lipsch_approx}
 \end{equation}
 where we neglected the terms of $O(||H||^2)$. Now, using triangular inequality %$||A+B|| \leq ||A|| + ||B||$,
 \[
 \leq || \Omega ss^T \Omega H \Omega|| + ||\Omega H \Omega ss^T\Omega||
 \]
 using sub-multiplicative property of the norm $||AB|| \leq ||A||||B||$,
 \[
 \leq ||ss^T||  \;  || \Omega ||^3 || H || = ||s||^2 || \Omega ||^3 || H ||
 \]
 since $|| \Omega || = || (I+L)^{-1}|| = \lambda_{\mathrm{max}} ((I+L)^{-1})= 1/(1+\lambda_{\mathrm{min}}(L))=1$, the minimum eigenvalue of a laplacian matrix is $0$, and $ss^T$ has a unique eigenvalue different from zero equal to $||s||^2$, the Lipschitz constant is
 \[
 \frac{||\partial f(L + H) - \partial f(L)||}{||H||} \leq ||s||^2
 \] \qedsymbol{}

\textit{Remark}: Notice that the missing term in Eq. \ref{eq:lipsch_approx}, i.e. $\Omega H \Omega ss^T \Omega H \Omega$, has a norm which is upper bounded by $O(||H||^2)$ using sub-multiplicativity. Moreover, the term contains $||-\Omega||=\lambda_{\mathrm{min}}((I+L)^{-1})=1/(1+\lambda_{\mathrm{max}}(L))$; since the maximum eigenvalue of a laplacian matrix is bounded from above by twice the maximum degree of the graph, this multiplicative term goes to zero as the size of network grows.

\spara{Algorithm.}
Algorithm \ref{alg:algorithm} has the following steps. It starts by initializing the solution uniformly and projecting it into the feasible set (lines 1-2). It then stores the learning rate $\eta$ and initializes an empty set of objective values. While the reduction in the objective value is greater than an input threshold $\delta$, the algorithm performs the following steps. In line 7, it invokes the Biconjugate Gradient (BiCG) algorithm to solve the linear system $(I+L)z=s$, which implies that the gradient in Eq. \ref{eq:gradient} is $(I+L)^{-1}ss^T(I+L)^{-1}=zz^T$ (line 8). The algorithm then performs one step of gradient descent and projects the solution into the feasible set by invoking Alg. \ref{alg:proj} (lines 9-10). Finally, the objective value is stored using the solution of BiCG: $s^T(I+L)^{-1}s=s^Tz$.


\spara{Projection.}
To ensure that our updated solution satisfies the constraints, we need to project it onto the feasible set at each iteration. This gives rise to the following optimization problem:

\begin{equation}
\min_{L \in \mathcal{L}^{\subset G}_\mathbf{b}} ||\tilde{L}^{t+1}-L||,
\end{equation}

where $\tilde{L}^{t+1}$ is the updated solution obtained after one step of gradient descent, which may not satisfy the constraints.

One approach is to project the matrix onto the set of positive semidefinite (PSD) matrices by calculating its eigendecomposition, thresholding the eigenvalues ($\lambda_{\mathrm{min}}\geq0$), and then recomposing the matrix using its eigenvectors and eigenvalues. However, this requires Singular Value Decomposition algorithms \cite{plassman2005survey}, which have a polynomial time complexity with a power larger than 2.

Instead, we can exploit the doubly stochastic property of the adjacency matrix $A$, which implies that the corresponding Laplacian $L=I-A$ is diagonally dominant ($\sum_{i\neq j}a_{ij}\leq 1$) and therefore positive definite. This means that we only need a doubly stochastic adjacency matrix to satisfy the constraints. Starting from the updated matrix $A^{t+1}$ at iteration $t+1$, we can compute its doubly stochastic version in linear time using Sinkhorn's algorithm \cite{sinkhorn1967concerning}, which alternates the normalization by row and column. Sinkhorn's theorem guarantees the existence of a doubly stochastic matrix under certain conditions (having total support), such as having a positive diagonal, which in our problem corresponds to the personalized information that each user receives. More recent algorithms \cite{rontsis2020optimal} exploit the sparsity of the input matrix and employ ADMM to achieve faster convergence.

To incorporate this projection step into our algorithm, we introduce Alg. \ref{alg:proj}. We begin by setting all entries of the updated solution $\tilde{A}$ that correspond to non-existing edges to 0 (line 2), which corresponds to entries with a null differential in the matrix variable. We then normalize the matrix by row and column (lines 3-5) and return the corresponding Laplacian.


\begin{tcolorbox}[title=NOTE,colframe=red,]
This is what prevents us to reach the optimum, therefore it is important. I did not come up with something better than this projection and I am not sure if this paragraph is enough to support the design decisions. Comments?
\end{tcolorbox}

\spara{Initialization.}
To use the heuristic effectively, we must start with an initial solution within the feasible set that has low levels of polarization and disagreement. Although the solution $G=(v, \emptyset)$ may reduce disagreement at equilibrium, it is not technically feasible because nodes are not interacting with each other, furthermore, their opinions are not averaged to reduce polarization. While a randomly generated graph may be projected into the feasible set using Alg. \ref{alg:proj}, this process does not guarantee lower levels of polarization and disagreement than the input graph. In our experiments, we have found that a uniform initialization of the graph weights leads to equal or better results than the input graph. This finding aligns with the FJ opinion dynamics model, which predicts that interacting users tend to converge toward a consensus that reduces disagreement.

==> table.tex <==
\begin{tabular}{llllrrrrrr}
\toprule
{} &            network & distribution & polarization & \multicolumn{2}{l}{time} & \multicolumn{2}{l}{overall reduction} & \multicolumn{2}{l}{counterfactual reduction} \\
method & ADAM-LcGD &         SCS &         ADAM-LcGD &        SCS &                ADAM-LcGD &        SCS \\
\midrule
0 &           barabasi &     gaussian &          5.0 &  3.653054 &   72.985673 &         81.539908 &  79.899993 &                36.563252 &  30.927805 \\
1 &           barabasi &      uniform &          5.0 &  1.755449 &   47.905637 &         85.681159 &  85.604288 &                20.347446 &  19.919833 \\
2 &  dimacs10-football &     gaussian &          5.0 &  2.932125 &  121.374324 &         75.884303 &  72.925359 &                46.401008 &  39.824527 \\
3 &  dimacs10-football &      uniform &          5.0 &  2.315520 &   97.874518 &         83.219980 &  83.576593 &                28.558898 &  30.077178 \\
4 &              erdos &     gaussian &          5.0 &  1.725928 &   57.375044 &         76.770803 &  72.063518 &                40.966674 &  29.003855 \\
5 &              erdos &      uniform &          5.0 &  1.000510 &   16.908159 &         85.842551 &  85.578207 &                19.773310 &  18.275336 \\
6 &    political-books &     gaussian &          5.0 &  1.749489 &   24.015299 &         70.463632 &  61.006037 &                35.825758 &  15.277059 \\
7 &    political-books &      uniform &          5.0 &  1.256010 &   20.130963 &         84.394039 &  83.694679 &                22.585032 &  19.115781 \\
\bottomrule
\end{tabular}


==> table_directed_uniform.tex <==
\begin{tabular}{r|r|rrrr|rrrr|rrrr}
\toprule
\multicolumn{2}{c}{} &  \multicolumn{4}{c}{Counterfactual $\rho$ 
 ($\uparrow$ \textbf{better})} & \multicolumn{4}{c}{Overall $\rho$ ($\uparrow$ \textbf{better})} & \multicolumn{4}{c}{Time (sec)} \\ \cline{1-14}
 \multicolumn{1}{c}{} & \multicolumn{1}{|c|}{Polarity} & LcGD & neutral-view & oppo-view & pop & LcGD & neutral-view & oppo-view & pop & LcGD & neutral-view & oppo-view & pop \\
%\cline{1-14}
\multirow[c]{2}{*}{Albert-Barab\'{a}si} & 1 & \textbf{10.16} & 2.57 & 7.06 & -0.69 & \textbf{81.73} & 80.21 & 81.10 & 79.53 & 8.40 & 0.00 & 0.00 & 0.00 \\
 & 5.0 & \textbf{19.86} & 6.43 & 18.24 & -8.44 & \textbf{83.61} & 80.84 & 83.28 & 77.72 & 6.35 & 0.00 & 0.00 & 0.00 \\
\multirow[c]{2}{*}{brexit} & 1 & \textbf{28.24} & 19.37 & 20.45 & -1.62 & \textbf{82.16} & 79.96 & 80.23 & 74.74 & 43.08 & 0.02 & 0.04 & 0.02 \\
 & 5.0 & \textbf{28.24} & 19.37 & 20.45 & -1.62 & \textbf{82.16} & 79.96 & 80.23 & 74.74 & 38.09 & 0.02 & 0.06 & 0.03 \\
\multirow[c]{2}{*}{digg-friends} & 1 & \textbf{12.59} & 4.55 & 8.54 & -0.06 & \textbf{83.46} & 81.94 & 82.70 & 81.07 & 317.65 & 0.08 & 0.04 & 0.03 \\
 & 5.0 & \textbf{13.64} & -1.07 & 12.59 & -0.10 & \textbf{83.70} & 80.92 & 83.50 & 81.11 & 368.96 & 0.07 & 0.04 & 0.04 \\
\multirow[c]{2}{*}{ego-twitter} & 1 & \textbf{6.22} & 0.82 & 2.87 & -1.68 & \textbf{82.93} & 81.95 & 82.32 & 81.49 & 63.48 & 0.00 & 0.00 & 0.00 \\
 & 5.0 & \textbf{6.21} & -1.56 & 4.73 & -1.79 & \textbf{83.76} & 82.42 & 83.51 & 82.38 & 48.23 & 0.00 & 0.00 & 0.00 \\
\multirow[c]{2}{*}{epinions} & 1 & \textbf{15.91} & 6.89 & 10.74 & -0.32 & \textbf{83.69} & 81.94 & 82.69 & 80.54 & 243.38 & 0.03 & 0.02 & 0.02 \\
 & 5.0 & \textbf{16.86} & -1.23 & 15.72 & -0.24 & \textbf{83.79} & 80.26 & 83.57 & 80.46 & 220.29 & 0.03 & 0.03 & 0.03 \\
\multirow[c]{2}{*}{Erd\H{o}s-R\'{e}nyi} & 1 & \textbf{20.89} & 12.38 & 12.50 & -0.15 & \textbf{83.08} & 81.24 & 81.21 & 78.31 & 15.64 & 0.01 & 0.00 & 0.00 \\
 & 5.0 & \textbf{22.24} & 2.30 & 20.22 & -0.01 & \textbf{83.51} & 79.01 & 83.10 & 78.48 & 17.69 & 0.01 & 0.00 & 0.00 \\
\multirow[c]{2}{*}{facebook-wosn-wall} & 1 & \textbf{21.53} & 10.67 & 14.01 & 0.30 & \textbf{83.18} & 80.85 & 81.56 & 78.63 & 247.39 & 0.01 & 0.01 & 0.01 \\
 & 5.0 & \textbf{22.73} & -2.15 & 21.40 & 0.06 & \textbf{83.53} & 78.23 & 83.25 & 78.70 & 239.66 & 0.01 & 0.01 & 0.01 \\
\multirow[c]{2}{*}{flickr-growth} & 1 & \textbf{14.83} & 3.70 & 9.75 & -0.48 & \textbf{83.83} & 81.72 & 82.86 & 80.92 & 2\,904.03 & 2.02 & 0.70 & 1.31 \\
 & 5.0 & \textbf{16.04} & -5.54 & 14.93 & -0.66 & \textbf{84.08} & 79.98 & 83.87 & 80.91 & 2\,919.71 & 2.10 & 0.81 & 1.01 \\
\multirow[c]{2}{*}{munmun} & 1 & \textbf{6.88} & 1.00 & 3.36 & -0.13 & \textbf{83.43} & 82.38 & 82.80 & 82.18 & 49.47 & 0.05 & 0.02 & 0.02 \\
 & 5.0 & \textbf{7.50} & -0.91 & 5.98 & -0.06 & \textbf{83.52} & 82.03 & 83.25 & 82.18 & 368.91 & 0.03 & 0.03 & 0.03 \\
\multirow[c]{2}{*}{sbm} & 1 & \textbf{27.53} & 17.03 & 17.40 & 0.13 & \textbf{83.09} & 80.64 & 80.72 & 76.69 & 30.76 & 0.00 & 0.01 & 0.00 \\
 & 5.0 & \textbf{29.22} & 2.93 & 27.13 & -0.12 & \textbf{83.51} & 77.39 & 83.03 & 76.68 & 35.24 & 0.00 & 0.00 & 0.00 \\
\multirow[c]{2}{*}{soc-epinions1} & 1 & \textbf{14.86} & 5.66 & 9.55 & 0.12 & \textbf{83.60} & 81.83 & 82.57 & 80.76 & 258.03 & 0.02 & 0.01 & 0.01 \\
 & 5.0 & \textbf{16.08} & -2.88 & 14.81 & -1.50 & \textbf{83.96} & 80.33 & 83.72 & 80.60 & 272.88 & 0.02 & 0.01 & 0.01 \\
\multirow[c]{2}{*}{vaxNoVax} & 1 & \textbf{29.76} & 23.19 & -3.66 & -0.42 & \textbf{83.18} & 81.61 & 75.19 & 75.96 & 94.97 & 0.06 & 0.15 & 0.10 \\
 & 5.0 & \textbf{29.76} & 23.19 & -3.66 & -0.42 & \textbf{83.18} & 81.61 & 75.19 & 75.96 & 100.95 & 0.06 & 0.12 & 0.12 \\
\bottomrule
\end{tabular}


==> tikzlibrarybayesnet.code.tex <==
 % tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

